Implicit Neural Surface Deformation with Explicit Velocity Fields

In this work, we introduce the first unsupervised method that simultaneously predicts time-varying neural implicit surfaces and deformations between pairs of point clouds. We propose to model the point movement using an explicit velocity field and directly deform a time-varying implicit field using the modified level-set equation. This equation utilizes an iso-surface evolution with Eikonal constraints in a compact formulation, ensuring the integrity of the signed distance field. By applying a smooth, volume-preserving constraint to the velocity field, our method successfully recovers physically plausible intermediate shapes. Our method is able to handle both rigid and non-rigid deformations without any intermediate shape supervision. Our experimental results demonstrate that our method significantly outperforms existing works, delivering superior results in both quality and efficiency.

==> figure_tex/4d_dress.tex <==
\begin{table}[t]
    \footnotesize
    \centering
    % \addtolength{\tabcolsep}{-3pt}
    \begin{tabular}{lcccc}
        \specialrule{.1em}{.05em}{.05em} 
        \toprule
       
         &  CD \tiny{$(\times 10^4)\downarrow$} & HD \tiny{$(\times 10^2)\downarrow$} & \SAstd \tiny{$(\times 10)\downarrow$}
         &  P-RMSE \tiny{$(\times 10)\downarrow$} \\ 
        \midrule
     
        NFGP~\cite{yang2021geometry}            & 0.272 & \textbf{0.025} & 0.075 & \xmark  \\
        LipMLP~\cite{liu2022learning}          & 14.99 & 2.125 & 1.252 & \xmark \\
        NISE~\cite{Novello2023neural}            & 6.588 & 2.167 & 0.321 & \xmark \\
         Ours & \textbf{0.270} & 0.047 & \textbf{0.023} & 0.024  \\
        \bottomrule
    \end{tabular}
    \caption{We evaluate our method with comparison methods on the~\textbf{4d-Dress}~\cite{wang20244ddress} dataset where the intermediate shapes are given. We report the average Chamfer Distance (CD) and Hausdorff Distance (HD) over 5 interpolated meshes. We also report the standard deviation of the surface area \SAstd~to indicate the changes in mesh-area over the deformation. Moreover, to evaluate our velocity field, we compute the per-point Euclidean distance as Root Mean Square Error (P-MSE) over the ground truth meshes. For the comparison methods that cannot compute the per-point distance error, we mark it as \xmark. 
    }
    \label{tab:4d_dress}
    \vspace*{-2mm}
\end{table}

